Scalable and Effective Negative Sample Generation for Hyperedge Prediction

Hyperedge prediction is crucial in hypergraph analysis for understanding complex multi-entity interactions in various web-based applications, including social networks and e-commerce systems. Traditional methods often face difficulties in generating high-quality negative samples due to the imbalance between positive and negative instances. To address this, we present the Scalable and Effective Negative Sample Generation for Hyperedge Prediction (SEHP) framework, which utilizes diffusion models to tackle these challenges. SEHP employs a boundary-aware loss function that iteratively refines negative samples, moving them closer to decision boundaries to improve classification performance. SEHP samples positive instances to form sub-hypergraphs for scalable batch processing. By using structural information from sub-hypergraphs as conditions within the diffusion process, SEHP effectively captures global patterns. To enhance efficiency, our approach operates directly in latent space, avoiding the need for discrete ID generation and resulting in significant speed improvements while preserving accuracy. Extensive experiments show that SEHP outperforms existing methods in accuracy, efficiency, and scalability, representing a substantial advancement in hyperedge prediction techniques. Our code is available here.

==> t__fig_diffusion.tex <==


%  68.6+63.12+33.21+107



\begin{figure*}[htbp]
    \centering
    \subfigure[Cora]{\includegraphics[width=0.21\textwidth]{diffusion_step/CoauthorshipCora_AUROC}    }
    \subfigure[DBLP]{\includegraphics[width=0.21\textwidth]{diffusion_step/CoauthorshipDBLP_AUROC}    }
    \subfigure[Citeseer]{\includegraphics[width=0.21\textwidth]{diffusion_step/CocitationCiteseer_AUROC}    }
    \subfigure[NDC\_class]{\includegraphics[width=0.21\textwidth]{diffusion_step/NDC_classes_AUROC}    }
    \caption{Effect of diffusion steps on AUROC for SEHP across four datasets: Cora, DBLP, Citeseer, and NDC\_classes.}
    \label{fig:auc_diffusion_step}
\end{figure*}

\begin{figure*}[htbp]
    \centering
    \subfigure[Cora]{\includegraphics[width=0.21\textwidth]{diffusion_step/CoauthorshipCora_Precision}    }
    \subfigure[DBLP]{\includegraphics[width=0.21\textwidth]{diffusion_step/CoauthorshipDBLP_Precision}    }
    \subfigure[Citeseer]{\includegraphics[width=0.21\textwidth]{diffusion_step/CocitationCiteseer_Precision}    }
    \subfigure[NDC\_class]{\includegraphics[width=0.21\textwidth]{diffusion_step/NDC_classes_Precision}    }
    \caption{Effect of diffusion steps on precision for SEHP across four datasets: Cora, DBLP, Citeseer, and NDC\_classes.}
    \label{fig:ap_diffusion_step}
\end{figure*}



==> t__fig_diffusion_epre.tex <==


%

% diffusion_step/CoauthorshipCora_AP
% diffusion_step/CoauthorshipDBLP_AP
% diffusion_step/CocitationCiteseer_AP
% diffusion_step/NDC_classes_AP




%

% diffusion_step_epre/CoauthorshipCora_AP
% diffusion_step_epre/CoauthorshipDBLP_AP
% diffusion_step_epre/CocitationCiteseer_AP
% diffusion_step_epre/NDC_classes_AP

%  68.6+63.12+33.21+107


\begin{figure*}[htbp]
    \centering
    \subfigure[Cora]{\includegraphics[width=0.21\textwidth]{diffusion_step_epre/CoauthorshipCora_AUROC}    }
    \subfigure[DBLP]{\includegraphics[width=0.21\textwidth]{diffusion_step_epre/CoauthorshipDBLP_AUROC}    }
    \subfigure[Citeseer]{\includegraphics[width=0.21\textwidth]{diffusion_step_epre/CocitationCiteseer_AUROC}    }
    \subfigure[NDC\_class]{\includegraphics[width=0.21\textwidth]{diffusion_step_epre/NDC_classes_AUROC}    }
    \caption{Effect of diffusion steps on AUROC  for the SEHP-epre across four datasets: Cora, DBLP, Citeseer, and NDC\_classes.}
    \label{fig:auc_diffusion_step_epre}
\end{figure*}



\begin{figure*}[htbp]
    \centering
    \subfigure[Cora]{\includegraphics[width=0.21\textwidth]{diffusion_step_epre/CoauthorshipCora_Precision}    }
    \subfigure[DBLP]{\includegraphics[width=0.21\textwidth]{diffusion_step_epre/CoauthorshipDBLP_Precision}    }
    \subfigure[Citeseer]{\includegraphics[width=0.21\textwidth]{diffusion_step_epre/CocitationCiteseer_Precision}    }
    \subfigure[NDC\_class]{\includegraphics[width=0.21\textwidth]{diffusion_step_epre/NDC_classes_Precision}    }
    \caption{Effect of diffusion steps on precision for the SEHP-epre across four datasets: Cora, DBLP, Citeseer, and NDC\_classes.}
    \label{fig:ap_diffusion_step_epre}
\end{figure*}


==> y_Hyper-parameters_Sensitivity.tex <==
\input{t__fig_diffusion}
\input{t__fig_diffusion_epre}




\subsubsection{Hyper-parameters Sensitivity}
We further investigate the effect of denoise steps on SEHP, where the number of denoise steps can be selected from [10, 20, 30, \ldots, 90, 100]. The results are shown in Figure~\ref{fig:auc_diffusion_step} for AUROC and Figure~\ref{fig:ap_diffusion_step} for Precision. From Figure~\ref{fig:auc_diffusion_step}, it is evident that the SEHP model maintains a high AUROC across different diffusion steps, with the highest values consistently achieved around the 30 to 50 denoise step range for most datasets. Specifically, for the Cora and DBLP datasets, AUROC remains relatively stable, while for Citeseer and NDC\_classes, there are more noticeable variations, particularly at lower diffusion steps. As shown in Figure~\ref{fig:ap_diffusion_step}, the precision for SEHP shows a trend similar to that of AUROC, with optimal performance typically within the 30 to 50 denoise step range. The precision values are relatively stable for Cora and DBLP, while Citeseer and NDC\_classes exhibit more variability. This indicates that the diffusion step is a crucial hyperparameter for optimizing SEHP's performance, with both AUROC and Precision maximized within the 30 to 50 range.


We also investigated the effect of denoise steps on SEHP-epre. The results are shown in Figure~\ref{fig:auc_diffusion_step_epre} for AUROC and Figure~\ref{fig:ap_diffusion_step_epre} for precision. SEHP-epre experiences more significant fluctuations in AUROC with varying diffusion steps, indicating that the absence of node ID extraction makes the model more sensitive to the choice of diffusion steps, potentially leading to less stable performance. Figure~\ref{fig:ap_diffusion_step_epre} shows that SEHP-epre also exhibits variability in Precision with different diffusion steps, similar to the AUROC results. Despite these fluctuations, SEHP-epre still maintains a competitive performance level, showcasing its ability to handle negative hyperedge representations directly. Overall, SEHP-epre demonstrates a greater sensitivity to the number of diffusion steps compared to the full SEHP model, highlighting the importance of incorporating node ID extraction for enhanced stability. However, the direct use of generated negative hyperedge representations in SEHP-epre provides a simpler and potentially more flexible approach in scenarios where node ID extraction might be less feasible.

==> y_method_negative_generator.tex <==
\subsection{Negative Hyperedge Generator}
\label{sec:negativeSampling}
The primary objective of the generator in hyperedge prediction is to generate high-quality negative samples, which significantly differs from conventional generator methods (e.g., in computer vision~\cite{10447191,Chen_2023_ICCV,pmlr-v202-bao23a} and NLP~\cite{NEURIPS2022_1be5bc25,he-etal-2023-diffusionbert,NEURIPS2023_35b5c175}), where the goal is to generate high-quality positive samples. If the generator is too weak, it produces only trivial negative hyperedge samples, which are ineffective for training the discriminator. Conversely, if the generator is too powerful and generates positive hyperedge samples from the target set, it fails to provide the true negative samples. 


Diffusion models have showcased substantial capabilities in sample generation. Nonetheless, adapting these models for negative hyperedge generation presents distinct challenges: (1) \textbf{Defining an effective ``good'' negative sample is problematic as diffusion models are fundamentally designed to produce well-defined, high-quality positive samples, rather than negative ones}; (2) \textbf{Diffusion models operate in a continuous space, while negative sampling for this task necessitates operations in a discrete space}. For scalability, the diffusion process should be constrained to the batched sub-hypergraph space, sampled as described in~\ref{Positive Hyperedges Sampling for Batch Processing}. However, as training progresses, the composition of the sub-hypergraph varies with each batch change. (3) \textbf{This variability in sub-hypergraph composition is not inherently recognized by diffusion models, potentially impacting the quality of generated negative samples}.

In the following sub-sections, we will explore strategies to effectively integrate diffusion models into the negative hyperedge generation process, addressing these challenges to improve model performance and scalability.

\subsubsection{Diffusion-Based Negative Hyperedge Representation Generation}


Conventionally, diffusion methods~\cite{NEURIPS2020_4c5bcfec,NEURIPS2021_49ad23d1} have two phases: adding noise and denoising. First, noise is iteratively added to the original sample until it becomes random noise, thus creating labeled data for training. Then, the denoising process aims to iteratively recover the noised data to the original sample. However, in hyperedge prediction, there is no clear notion of what constitutes a good negative sample, so there is no original sample to start with. Instead, the score predicted by the classifier can be used as a signal to supervise the denoising process. Given a negative hyperedge representation at time $t$, a new negative hyperedge representation at time $t+1$ can be generated by denoising the current negative hyperedge representation. The signal for denoising is ${\text{score}_{\text{hyperedge}}^{t} < \text{score}_{\text{hyperedge}}^{t+1}}$, and the process of denoising is defined as follows:
\begin{equation}
    \mathbf{h}_{e}^{t+1} = \text{Denoise}(\mathbf{h}_{e}^{t})
    \label{eq:denoise}
\end{equation}


where $\mathbf{h}_{e}^{t}$ is the negative hyperedge representation at time $t$, and $\mathbf{h}_{e}^{t+1}$ is the negative hyperedge representation at time $t+1$. Here, $\mathbf{h}_{e}^{0} = \mathbf{h}_{\hat{e}}^{p}$, where $\hat{e}^{p}$ is a representation of a positive hyperedge $\hat{e}$. The denoising process can be any neural network, such as a MLP, recurrent neural network~\cite{SIP-2022-0023}, or graph neural network~\cite{9835563,10184723,10184514}. In this work, a MLP is used for the denoising process.



\subsubsection{Conditional Denoising for Controlled Diffusion}
As training progresses, the composition of the sub-hypergraph varies with each batch change, a factor not inherently recognized by traditional diffusion models. To enhance the control over the direction of the diffusion process, we introduce a conditional mechanism into the denoising phase. This adjustment addresses the issue that information from a single positive hyperedge is often insufficient for generating high-quality negative samples. Instead, the structural information of the sub-hypergraph, which encapsulates more comprehensive global data, is utilized. 

The conditional mechanism thus incorporates the structural information of the sub-hypergraph as an additional input. This integration, when combined with the candidate hyperedge representation, facilitates the generation of an enhanced negative hyperedge representation. The formal definition of the conditional denoising process is as follows:
\begin{equation}
    \mathbf{h}_{e}^{t} = \text{Denoise}(\mathbf{h}_{e}^{t-1}, \mathbf{h}_{structure}^{sub})
    \label{eq:conditional_denoise}
\end{equation}
where $\mathbf{h}_{structure}^{sub}$ is the structural information of the sub-hypergraph, and $\mathbf{h}_{e}^{t}$ is the negative hyperedge representation at time $t$. $\mathbf{h}_{structure}^{sub}$ can be obtained by reading out the node embeddings of the sub-hypergraph. The readout process can be any neural network, such as sum, mean, max, or attention-based readout. In this work, an average readout process is used to obtain the structural information of the sub-hypergraph. The whole process is illustrated in the component "Negative Representation Generation" of Figure~\ref{fig:framework}.

\begin{figure*}[htbp]
\centerline{\includegraphics{z_edge_representation}}
\caption{Framework of Diffusion Based Negative Hyperedge Generation for Hyperedge Prediction, but using generated hyperedge embedding directly. This can be put in appendix.}
\label{fig:framework_edge_representation}
\end{figure*}



\subsubsection{Node ID Extraction}
In hyperedge prediction using diffusion models, the transition from a continuous representation to a discrete set of node IDs presents a critical challenge. While the diffusion component operates efficiently in a continuous space, the final goal in hyperedge prediction is to accurately identify which nodes form a negative hyperedge, which requires discrete outputs. Therefore, after obtaining the negative hyperedge representation through diffusion, it is essential to map this continuous data back into discrete node IDs to form a viable negative hyperedge.

This mapping process involves combining the negative hyperedge representation with the embeddings of candidate nodes from the sub-hypergraph. By applying a machine learning model, typically MLP, we can estimate the probability of each node being part of the negative hyperedge. The formal definition of the Node ID extraction process is as follows:
\begin{equation}
    e_t = \{\hat{v}_1^{sub}, \hat{v}_2^{sub}, \ldots, \hat{v}_k^{sub}\} = \text{Topk}(p_{v_1}, p_{v_2}, \ldots, p_{v_n})
    \label{eq:node_id_extraction}
\end{equation}
\[
p_{v_i} = \text{MLP}(\mathbf{h}_{e}^t, \mathbf{v}_i)
\]
where $e_t$ represents the negative hyperedge at time $t$, $\hat{v}_i^{sub}$ is the $i$-th node in the negative hyperedge, and $p_{v_i}$ is the probability of node $v_i$ being part of the negative hyperedge, calculated based on the MLP output. The MLP is designed with a sigmoid activation function to ensure that the output probabilities are bounded between 0 and 1.

This process not only translates the continuous representation produced by the diffusion process into a usable set of node IDs but also ensures that the most likely candidates are selected to form the hyperedge, based on their computed probabilities. This method effectively bridges the gap between the generative capabilities of diffusion models and the discrete nature of hyperedge prediction tasks, thus enhancing the overall performance and accuracy of the system.




% \subsection{Negative Hyperedge Generator}
% \label{sec:negativeSampling}
% \subsubsection{Challenges}
% The primary objective of the generator in hyperedge prediction is to generate high-quality negative samples, which significantly differs from conventional generator methods (e.g., in computer vision~\cite{10447191,Chen_2023_ICCV,pmlr-v202-bao23a} and NLP~\cite{NEURIPS2022_1be5bc25,he-etal-2023-diffusionbert,NEURIPS2023_35b5c175}), where the goal is to generate high-quality positive samples. 

% \textbf{Challenge 1: Balancing the Generator's Effectiveness.}  
% If the generator is too weak, it produces only trivial negative hyperedge samples, which are ineffective for training the discriminator. Conversely, if the generator is too powerful and generates positive hyperedge samples from the target set, it fails to provide the true negative samples. 

% \textbf{Challenge 2: Producing Negative Samples Near the Decision Boundary.}  
% Since hyperedge prediction is a binary classification task, another critical challenge is ensuring that the generator produces negative samples that are near the decision boundary. This is crucial for effectively training the discriminator to distinguish between positive and negative samples, yet it is a difficult requirement to meet.

% \textbf{Challenge 3: Selecting Candidate Nodes and Ensuring Scalability.}  
% Identifying candidate nodes for generating negative hyperedges in large hypergraphs presents another significant challenge. For large hypergraphs, sampling a sub-hypergraph for batch processing is a common approach. However, the varying number of nodes in different batches makes it impractical to use an MLP with a fixed output size to predict the probability for each node in the current batch. Hence, finding scalable and flexible methods for candidate node selection is essential to adapt to changing node numbers and maintain efficiency in large hypergraphs.

% Addressing these challenges requires innovative approaches to ensure effective training and scalability in hyperedge prediction tasks.

% \subsubsection{Diffusion-Based Negative Hyperedge Representation Generation}

% Conventionally, diffusion methods~\cite{NEURIPS2020_4c5bcfec,NEURIPS2021_49ad23d1} have two phases: adding noise and denoising. First, noise is iteratively added to the original sample until it becomes random noise, thus creating labeled data for training. Then, the denoising process aims to iteratively recover the noised data to the original sample. However, in hyperedge prediction, there is no clear notion of what constitutes a good negative sample, so there is no original sample to start with. Instead, the score predicted by the classifier can be used as a signal to supervise the denoising process. Given a negative hyperedge representation at time $t$, a new negative hyperedge representation at time $t+1$ can be generated by denoising the current negative hyperedge representation. The signal for denoising is ${score}^{t}_{hyperedge} < {score}^{t+1}_{hyperedge}$, and the process of denoising is defined as follows:
% \begin{equation}
%     \mathbf{h}_{e}^{t+1} = \text{Denoise}(\mathbf{h}_{e}^{t})
%     \label{eq:denoise}
% \end{equation}
% where $\mathbf{h}_{e}^{t}$ is the negative hyperedge representation at time $t$, and $\mathbf{h}_{e}^{t+1}$ is the negative hyperedge representation at time $t+1$. Here, $\mathbf{h}_{e}^{0} = \mathbf{h}_{\hat{e}}^{p}$, where $\hat{e}^{p}$ is a representation of a positive hyperedge $\hat{e}$. The denoising process can be any neural network, such as a feedforward neural network, recurrent neural network, or graph neural network. In this work, a feedforward neural network is used for the denoising process.

% \subsubsection{Conditional Denoising for Controlled Diffusion}

% To better control the direction of the diffusion process, a conditional mechanism is introduced to the denoising process. When generating a negative hyperedge, the information from a single positive hyperedge is insufficient; the structural information of the sub-hypergraph provides more comprehensive global information. Consequently, the conditional mechanism incorporates the structural information of the sub-hypergraph as an additional input, which, combined with the candidate hyperedge representation, generates the new negative hyperedge representation. The formal definition of the conditional denoising process is as follows:
% \begin{equation}
%     \mathbf{h}_{e}^{t} = \text{Denoise}(\mathbf{h}_{e}^{t-1}, \mathbf{h}_{structure}^{sub})
%     \label{eq:conditional_denoise}
% \end{equation}
% where $\mathbf{h}_{structure}^{sub}$ is the structural information of the sub-hypergraph, and $\mathbf{h}_{e}^{t}$ is the negative hyperedge representation at time $t$. $\mathbf{h}_{structure}^{sub}$ can be obtained by reading out the node embeddings of the sub-hypergraph. The readout process can be any neural network, such as sum, mean, max, or attention-based readout. In this work, an average readout process is used to obtain the structural information of the sub-hypergraph. The whole process is illustrated in the component "Negative Representation Generation" of Figure~\ref{fig:framework}.

% \begin{figure*}[htbp]
% \centerline{\includegraphics{z_edge_representation}}
% \caption{Framework of Diffusion Based Negative Hyperedge Generation for Hyperedge Prediction, but using generated hyperedge embedding directly. This can be put in appendix.}
% \label{fig:framework_edge_representation}
% \end{figure*}

% \subsubsection{Node ID Extraction}

% Naturally, the diffusion component can only operate in continuous space. However, for existing hyperedge prediction work, the negative hyperedge generator returns a discrete subset of node IDs. Therefore, after obtaining the negative hyperedge representation through diffusion, it is necessary to extract the node IDs from the generated negative hyperedge representation to form a negative hyperedge. All nodes from the sub-hypergraph can be considered candidates. The negative hyperedge representation is combined with the candidate node embeddings to predict the probability of each node being part of the target negative hyperedge. The top k nodes with the highest probabilities are selected to form the negative hyperedge, where k is the size of the given positive hyperedge $\hat{e}$. The formal definition of the node ID extraction process is as follows:
% \begin{equation}
%     e_t = \{v_{\hat{1}}^{sub}, v_{\hat{2}}^{sub}, ..., v_{\hat{k}}^{sub}\} = \text{Topk}(p_{v_1}, p_{v_2}, ..., p_{v_n}) 
%     \label{eq:node_id_extraction}
% \end{equation}
% \[
% p_{v_i} = \text{MLP}(\mathbf{h}_{e}^{t}, \mathbf{v}_i)
% \]
% where $e_t$ is the negative hyperedge at time $t$, $v_{\hat{i}}^{sub}$ is the $i$-th node in the negative hyperedge, $p_{v_i}$ is the probability of node $v_i$ being in the negative hyperedge, and $\mathbf{v}_i$ is the node embedding of node $v_i$. The MLP is a feedforward neural network with a sigmoid activation function.








